Through the Fairness Lens: Experimental Analysis and Evaluation of Entity Matching

Entity matching (EM) is a challenging problem studied by different communities for over half a century. Algorithmic fairness has also become a timely topic to address machine bias and its societal impacts. Despite extensive research on these two topics, little attention has been paid to the fairness of entity matching. Towards addressing this gap, we perform an extensive experimental evaluation of a variety of EM techniques in this paper. We generated two social datasets from publicly available datasets for the purpose of auditing EM through the lens of fairness. Our findings underscore potential unfairness under two common conditions in real-world societies: (i) when some demographic groups are overrepresented, and (ii) when names are more similar in some groups compared to others. Among our many findings, it is noteworthy to mention that while various fairness definitions are valuable for different settings, due to EM's class imbalance nature, measures such as positive predictive value parity and true positive rate parity are, in general, more capable of revealing EM unfairness.

==> fn_archive.tex <==

\section{More on Fairness Notions}


\fn{discussion of pure fairness. This can also be summarized and moved to the intro/scope.}

\fn{Here, we talk a lot about "model". Since we are not considering rule-based matchers, can we minimize model references?}

There is no singular definition for fairness. It all  depends on the type of task we target to solve and the numerous kinds of bias that can exist in data. Since our focus is mostly on auditing learning-based entity matching techniques, we provide a general overview of fairness definitions from the classification perspective. 
At a high level, fairness definitions can be viewed from three perspectives: group fairness, subgroup fairness, and individual fairness~\cite{fairmlbook}. 

The most granular notion of fairness is individual fairness that requires similar outcomes for similar individuals~\cite{dwork2012fairness}. 
The more popular perspectives of fairness for learning models,  group/subgroup fairness, require similar treatment for different  groups. 
A model satisfies some fairness constraints if the model has equal or similar performance (according to some fairness measure) on different subgroups. 
The focus of this paper is on group/subgroup fairness. 


\fn{if you feel this paragraph is out of place, we can summarize and move to the scope section in intro.}
Most of the group fairness measures belong to one of the four categories of {\em Independence}, {\em Separation}, {\em Sufficiency}, and {\em Causation}~\cite{fairmlbook,asudeh2020fairly}.
A model satisfies {\em independence} if its outcome is independent from the sensitive attributes. Measures such as {\em Statistical Parity} fall under this category.
{\em Separation} is satisfied when the outcome of the model is independent from the sensitive attribute(s) conditioned on the target variable. The well-known measure in this category is {\em Equalized Odds}~\cite{hardt2016equality}.
On the other hand, \textit{Sufficiency} is satisfied if under the same model outcomes, sensitive attribute(s) and the true outcome are independent and it can be measured with \textit{Predictive Parity}. 
\textit{Causation} is however somehow different from the rest and focuses on the causal relationship between attributes for instance when  an attribute $A$ affects attribute $B$, which in turn affects attribute $C$. Domain experts are required to analyze a model in terms of Causality. Since we only assume access to a matcher's decisions and true labels and not the whole data set, we choose to not to focus on Causal fairness in our audit.

Falling in between individual and group fairness, subgroup fairness (also known as intersectional fairness) metrics measure fairness (according to the above definitions) when  groups are defined over intersection of values of multiple sensitive attributes (e.g. {\tt white~male}, {\tt white~female}, {\tt black~male}, and {\tt black~female}). 

Regardless of the definition of fairness chosen to evaluate a model, there are challenges and domain-specific choices that need to be taken care of. 
Except for Equal Employment Opportunity Commission’s 80\% rule~\cite{EEOC} that has been formalised as a bias measure, called Disparate Impact, there are no official guidelines for other measures. As a result, a model should be audited for groups of interest based on user-provided thresholds.  
Finding the subgroups for which a model is unfair is challenging. 
One reason is that a model can be fair with respect to any group individually but unfair towards a subgroup when fair groups are combined (e.g. a model that is fair both to {\tt\small female} and {\tt\small black}, can be unfair to {\tt\small female black} subgroup). Identifying groups to which a model is discriminatory is particularly challenging due to the large space of possible subgroups. 



\subsubsection{Fairness Metrics}
% \label{sec:emfairmeasures}

Depending on the context of an entity matching task at hand, proper fairness measures should be employed. More precisely, the adopted fairness measures depend on the importance of TPs, FPs, FNs, and TNs in the problem context and how forgiving we can be towards each. 

We note that  some measures cannot be applied in pairwise fairness scenarios where conceptually the equality of groups restricts matching results. 
 In some scenarios, two entities with different  groups can never be considered as a {\em match} in the ground-truth. 
For instance, in a matching task defined between {\em DBLP} and {\em ACM} publications, two entities with different venues (after standardization) and years are  never a true {\em match}. More concretely, when pairwise fairness is evaluated on subgroups with non-overlapping groups, TPs and FNs are always zero, therefore, fairness measures that rely on TPs and FNs become inapplicable. 

In what follows, we present a suite of fairness measures, based on notions of fairness in classification~\cite{fairmlbook} and repurposed for entity matching,  for auditing an  entity matcher $\mathcal{M}$ with respect to a set $\gee$ of $k$-combination subgroups. Let $h(e,e^\prime)$ be the output of  matcher $\mathcal{M}$  ({\em match} (`M') or {\em non-match} (`N')) and $y$ be the ground-truth on entities $e$ and $e^\prime$.  
\begin{itemize}[leftmargin=*]
    \item \textbf{Accuracy Parity (AP)} equalizes matchers's accuracy across different subgroups:
    \begin{equation}
    \label{equation:acc}
    \forall g_i\in \gee, Pr(h(e,e^\prime)=y\vert g_i) \simeq Pr(h(e,e^\prime)=y)
    \end{equation}
    Accuracy parity is a useful measure in the contexts where the impact of FPs and FNs are similar. This measure extends to both \textit{single} and \textit{pairwise} fairness definitions.
    Alternatively, instead of accuracy, one can consider the {\bf misclassification rate parity}:
    \begin{equation}
    \label{equation:mis}
    \forall g_i\in \gee, Pr(h(e,e^\prime)\neq y~\vert~g_i) \simeq Pr(h(e,e^\prime)\neq y)
    \end{equation}
    
    \item \textbf{Statistical Parity (SP)} makes the independence assumption of the matcher from  groups ($h\,\bot\, \gee$). 
    Under statistical parity~\cite{dwork2012fairness}, the probability of a matcher outcome is equal or similar across different groups:
    \begin{equation}
    \label{equation:dp}
    \forall g_i\in \gee, Pr(h(e,e^\prime)=`M\textrm'~\vert~g_i) \simeq Pr(h(e,e^\prime)=`M\textrm')
    \end{equation}
    Statistical parity is not an applicable fairness measure in deduplication tasks using entity matching since equal probability of getting a match given a subgroup may not be meaningful, however,  this measure is useful for entity matching in table joins. Furthermore, this measure extends to both \textit{single} and \textit{pairwise} fairness definitions.
    % \vspace{2mm}
    
    \item \textbf{True Positive Rate Parity (TPRP)} also known as \textit{Equal Opportunity} or \textit{Sensitivity} is a practical measure when predicting the positive outcome correctly is crucial and FPs are not costly:
    \begin{equation}
    \label{equation:tpr}
     \forall g_i\in \gee, Pr(h(e,e^\prime) = `M\textrm'\vert g_i, y=`M\textrm') \simeq Pr(h(e,e^\prime) = `M\textrm' \vert y=`M\textrm') 
    \end{equation}
    This measure is only meaningful for \textit{single} fairness and is not definable in \textit{pairwise} fairness. The reason is that  when the  groups of  two entities to be matched are different, it is impossible for the ground-truth to be \textit{match}, therefore number of TPs is always zero.
    % \vspace{2mm}
    
    \item \textbf{False Positive Rate Parity (FPRP)} is a useful measure in contexts that minimizing costly FPs matter most:
    \begin{equation}
    \label{equation:fpr}
     \forall g_i\in \gee, Pr(h(e,e^\prime) = `M\textrm' \vert g_i, y=`N\textrm') \simeq Pr(h(e,e^\prime) = `M\textrm' \vert  y=`N\textrm') 
    \end{equation}
    This measure extends to both \textit{single} and \textit{pairwise} fairness definitions.
    % \vspace{2mm}
    
    \item \textbf{False Negative Rate Parity (FNRP)} is a useful measure in contexts that FNs are costly and the overweighing source of error:
    \begin{equation}
    \label{equation:fnr}
     \forall g_i\in \gee, Pr(h(e,e^\prime) = `N\textrm' \vert g_i, y=`M\textrm') \simeq Pr(h(e,e^\prime) = `N\textrm' \vert  y=`M\textrm') 
    \end{equation}
    For the same reasons, this measure is also only meaningful for \textit{single} fairness and does not extend to \textit{pairwise} fairness. Entities with different  groups can not have a \textit{match} ground-truth. 
    
    \item \textbf{True Negative Rate Parity (TNRP)} also known as \textit{specificity} measures model's ability to correctly identify negative results:
    \begin{equation}
    \label{equation:tnr}
     \forall g_i\in \gee, Pr(h(e,e^\prime) = `N\textrm' \vert g_i, y=`N\textrm') \simeq Pr(h(e,e^\prime) = `N\textrm' \vert  y=`N\textrm') 
    \end{equation}
    This measure extends to both \textit{single} and \textit{pairwise} fairness definitions.
    % \vspace{2mm}
    
    \item \textbf{Equalized Odds (EO)} also known as \textit{Positive Rate Parity} is practical in contexts that correctly predicting positive outcomes and minimizing costly FPs are both of high importance:
    \begin{equation}
    \label{equation:eo}
    \begin{split}
    \forall g_i\in \gee, Pr(h(e,e^\prime)=`M\textrm'\vert g_i, y=`M\textrm') \simeq	 Pr(h(e,e^\prime)=`M\textrm'\vert  y=`M\textrm') 
    \\ 
    Pr(h(e,e^\prime)=`M\textrm'\vert g_i, y=`N\textrm') \simeq	 Pr(h(e,e^\prime)=`M\textrm'\vert  y=`N\textrm')
    \end{split}
    \end{equation}
    This measure is also only meaningful for \textit{single} fairness and does not extend to \textit{pairwise} fairness. 
    \item \textbf{Positive Predictive Value Parity (PPVP)} guarantees equal chance of success given positive prediction for all subgroups:
    \begin{equation}
    \label{equation:ppv}
    \forall g_i\in \gee, Pr(y=`M\textrm'\vert h(e,e^\prime)=`M\textrm', g_i) \simeq Pr(y=`M\textrm'\vert h(e,e^\prime)=`M\textrm')
    \end{equation}
    This measure is also only meaningful for \textit{single} fairness and does not extend to \textit{pairwise} fairness.
    % \vspace{2mm}
    
    \item \textbf{Negative Predictive Value Parity (NPVP)} ensures equal chance of success given negative prediction for all subgroups:
    \begin{equation}
    \label{equation:npv}
    \forall g_i\in \gee, Pr(y=`N\textrm'\vert h(e,e^\prime)=`N\textrm', g_i) \simeq Pr(y=`N\textrm'\vert h(e,e^\prime)=`N\textrm')
    \end{equation}
    This measure is also only meaningful for \textit{single} fairness and does not extend to \textit{pairwise} fairness.
    % \vspace{2mm}
    
    \item \textbf{False Discovery Rate Parity (FDRP)} makes the independence assumption of true match/non-match decision from subgroups, conditional on the {\em match} decision  ($y\,\bot\, \gee\vert ~h(e,e^\prime)=`M\textrm'$). 
    \begin{equation}
    \label{equation:fdr}
        \forall g_i\in \gee, Pr(y = `N\textrm' \vert g_i, h(e,e^\prime) = `M\textrm') \simeq Pr(y = `N\textrm' \vert  h(e,e^\prime) = `M\textrm') 
    \end{equation}
    This measure is also only meaningful for \textit{single} fairness and does not extend to \textit{pairwise} fairness.
    
    \item \textbf{False Omission Rate Parity (FORP)} makes the independence assumption of true match/non-match decision from subgroups, conditional on the {\em non-match} decision  ($y\,\bot\, \gee\vert ~h=0$). 
    \begin{equation}
    \label{equation:for}
        \forall g_i\in \gee, Pr(y = `M\textrm' \vert g_i, h(e,e^\prime) = `N\textrm') \simeq Pr(y = `M\textrm' \vert  h(e,e^\prime) = `N\textrm') 
    \end{equation}
    This measure is also only meaningful for \textit{single} fairness and does not extend to \textit{pairwise} fairness.
\end{itemize}

